MVImgNet2.0: A Larger-scale Dataset of Multi-view Images

MVImgNet is a large-scale dataset that contains multi-view images of ~220k real-world objects in 238 classes. As a counterpart of ImageNet, it introduces 3D visual signals via multi-view shooting, making a soft bridge between 2D and 3D vision. This paper constructs the MVImgNet2.0 dataset that expands MVImgNet into a total of ~520k objects and 515 categories, which derives a 3D dataset with a larger scale that is more comparable to ones in the 2D domain. In addition to the expanded dataset scale and category range, MVImgNet2.0 is of a higher quality than MVImgNet owing to four new features: (i) most shoots capture 360-degree views of the objects, which can support the learning of object reconstruction with completeness; (ii) the segmentation manner is advanced to produce foreground object masks of higher accuracy; (iii) a more powerful structure-from-motion method is adopted to derive the camera pose for each frame of a lower estimation error; (iv) higher-quality dense point clouds are reconstructed via advanced methods for objects captured in 360-degree views, which can serve for downstream applications. Extensive experiments confirm the value of the proposed MVImgNet2.0 in boosting the performance of large 3D reconstruction models. MVImgNet2.0 will be public at luyues.github.io/mvimgnet2, including multi-view images of all 520k objects, the reconstructed high-quality point clouds, and data annotation codes, hoping to inspire the broader vision community.

==> figures/exp_ingp2dgs.tex <==
\begin{figure}[t]
	\centering
	% \scriptsize
	\includegraphics[width=1\linewidth]{images/exp_vis_triplane.jpg}
    \vspace{-0.4cm}
	\caption{Qualitative results of Instant-NGP and 3DGS trained on real-world data with different camera poses estimated by the original manner in MVImgNet (MV1-Anno) and the advanced one (MV2-Anno).}
	\label{fig:exp_ingp2dgs}
 \vspace{-0.4cm}
\end{figure}

==> figures/old/fig_ablation.tex <==
\begin{figure}[htbp]
  \centering
  \vspace{3mm}
  \includegraphics[width=.98\linewidth]{images/fig_alation.png}
  \caption{Qualitative comparison between our diffusion-based and the optional GAN-based method (i.e., ours-pix2pix). For each case, the input image (a) is followed by the results generated by (b) ours-pix2pix and (c) ours.}
  \label{fig:exp_ablation}
  \vspace{8mm}
\end{figure}

==> figures/old/fig_compare.tex <==
\vspace{2mm}
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=.92\linewidth]{images/fig_compare.png}
  \caption{Qualitative comparison between ours and the state of the arts. For each row, the input image (a) is followed by the results generated by (b) BCNet~\cite{jiang2020bcnet}, (c) ClothWild~\cite{moon20223d}, (d) Deep Fashion3D~\cite{zhu2020deep}, (e) ReEF~\cite{zhu2022registering}, (f) our method, and (g) the ground truth.}
  \label{fig:exp_compare}
\end{figure*}



==> figures/old/fig_dataset_gallery.tex <==
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=.99\linewidth]{images/fig_dataset_gallery.png}
  \caption{The gallery of the representative examples sampled from MesoCloth3D. Each collected reference image is followed by the corresponding 3D garment model with meso-scale deformation, a rendered image from a random camera view, and a result generated by Canny-Conditional Stable Diffusion models.}
  \label{fig:data_gallery}
\end{figure*}

==> figures/old/fig_dataset_pipeline.tex <==
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=.99\linewidth]{images/fig_dataset_pipeline.png}
  \caption{The pipeline of our novel data generation strategy. \textbf{3D Garment Crafting:} Given a ``Collected Image'', we utilize PyMAF~\cite{pymaf2021,pymafx2023} to estimate SMPL body. Eight artists are then tasked with creating ``T-pose Garment'' shapes by deforming a predefined ``Template'' to match the T-pose body predicted by PyMAF. Then the SMPL's Linear Blend Skinning (LBS) is extended to the T-pose garment to obtain the ``Posed Garment''. Finally, the artists are further instructed to refine the posed garment to get the ``Crafted Garment'' while ensuring that meso-scale deformations closely match the collected images. \textbf{Data Augmentation:} We acquire rendered images of 3D garments with random camera views. These rendered images are processed through Canny-Conditional Stable Diffusion~\cite{zhang2023adding,mou2023t2i} to produce photorealistic images.}
  \label{fig:data_pipeline}
\end{figure*}

==> figures/old/fig_define.tex <==
% Use figure* for multi-column figure
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.99\linewidth]{images/fig_define.png}
    \caption{Looking into a clothed human (a), a garment geometry mainly comprises three levels of details: the  \textit{overall garment style}, i.e., T-pose shape (b), the \textit{meso-scale deformations}, i.e., medium- frequency deformation (c), and the \textit{surface details} (d).}
    \label{fig:define}
\end{figure}


==> figures/old/fig_dt.tex <==
% Use figure* for multi-column figure
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.98\linewidth]{images/fig_dt.png}
    \caption{An illustration of Meso-Scale Deformations Transfer. We can transfer meso-scale deformations (b) captured by \methodName to a well-designed garment (a) with arbitrary topology to get its deformed shapes (c).}
    \label{fig:dt}
    \vspace{-2mm}
\end{figure}


==> figures/old/fig_pipeline.tex <==
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=.99\linewidth]{images/fig_method.pdf}
  \caption{The pipeline of our proposed method. Given an RGB image, our method first estimates the T-pose garment shape $G({\mathrm{\alpha}})$ (Eq.~\ref{math:G}), then computes its pose-dependent meso-scale deformation $M_{\mathrm{P}}(\alpha, \beta, \theta)$ with the help of the predicted SMPL body (Eq.~\ref{math:TG}, Eq.~\ref{math:MP}), and finally captures its pose-independent meso-scale deformation $M_{\mathrm{G}}$ via a projected-conditioned denoising diffusion process.}
  \label{fig:method_pipeline}
\end{figure*}

==> figures/old/fig_result_gallery.tex <==
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=.92\linewidth]{images/fig_result_gallery.pdf}
  \caption{Result gallery of our method. Each image is followed by the reconstructed garment mesh.}
  \label{fig:result_gallery}
\end{figure*}

==> figures/old/fig_sde.tex <==
% Use figure* for multi-column figure
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.90\linewidth]{images/fig_sde.png}
    \caption{From left to right, each row contains (a) the input image, (b) the reconstructed mesh of Meso, (c) the normal map estimated by ICON, and (d) the surface details enhanced through normal map optimization.}
    \label{fig:sde}
    \vspace{8mm}
\end{figure}


==> figures/old/fig_te.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=.99\linewidth]{images/teaser.pdf}
    \caption{Examples of Text-Based Garment Editing. Given a garment (a1, b1) reconstructed by \methodName, we can carve its geometric details (a2, b2) via text2mesh~\cite{michel2022text2mesh} and generate its textures (a3, b3) with TEXTure~\cite{richardson2023texture}.
    %The garment shape reconstructed by \methodName can be futher carved geometric details through text2mesh~\cite{michel2022text2mesh}, and produce texture through TEXTure~\cite{richardson2023texture}.
    }
    \label{fig:te}
    \vspace{-3mm}
\end{figure}

==> paper/04_method.tex <==
\section{Method}
\label{sec:method}

Fig.~\ref{fig:method_pipeline} illustrates the framework of our garment reconstruction method. Given an RGB image, our method first estimates the T-pose garment shape (Sec.~\ref{sec:method_tg}), then computes its pose-dependent meso-scale deformation with the help of a predicted SMPL body (Sec.~\ref{sec:method_sd}), and finally captures its pose-independent meso-scale deformation via a conditional denoising diffusion process (Sec.~\ref{sec:method_sd}). Note that our method focuses on modeling meso-scale deformation and does not consider geometric details. Various existing methods have shown that geometric details can be easily recovered through normal map optimization, benefiting from the excellent performance of normal estimators, as demonstrated in Sec.~\ref{sec:application_detail}.

% show that a high-quality normal map significantly aids in recovering geometric details, benefiting from the excellent performance of normal estimators. 

% \subsection{Coarse Structure Reconstruction}
\subsection{T-pose Garment Estimation}
\label{sec:method_tg}
\paragraph{Unposed Garment Representation.} Various current works~\cite{jiang2020bcnet,bhatnagar2019multi,patel20tailornet,luo2023rabit} demonstrate that linear statistical models are able to represent the basic geometries of diverse shapes. We utilize and extend existing human body models~\cite{loper2023smpl,pavlakos2019expressive,romero2022embodied} to represent unposed (i.e., T-pose) garments. More specifically, we parameterize our garment on top of the widely recognized human model SMPL~\cite{loper2023smpl}. SMPL is a statistical parametric model that incorporates \textit{Body Shape Blend Shapes} (BSBS) and \textit{Body Pose Blend Shapes} (BPBS) to define an unposed body. Given the shape parameters ($\beta$) and pose parameters ($\theta$), SMPL can generate the unposed body mesh by
\begin{equation}
T_{\mathrm{B}}(\beta, \theta) = \mathbf{T}_{\mathrm{b}} + B_{\mathrm{s}}(\beta) + B_{\mathrm{p}}(\theta),
\end{equation}
where $\mathbf{T}_{\mathrm{b}} \in \mathbb{R}^{N_{\mathrm{B}} \times 3}$ is a body template mesh with $N_{\mathrm{B}}$ vertices. 
$B_{\mathrm{s}}(\beta) \in \mathbb{R}^{N_{\mathrm{B}} \times 3}$ denotes the shape-related displacements, while $B_{\mathrm{p}}(\beta) \in \mathbb{R}^{N_{\mathrm{B}} \times 3}$ models the pose-dependent correctiveness. 
To formulate our unposed garment model, we build a specific blending model as 
\begin{equation}
T_{\mathrm{G}}(\alpha, \beta, \theta) = G({\mathrm{\alpha}}) + \widetilde{B}_{\mathrm{s}}(G({\mathrm{\alpha}}), \beta) 
+ \widetilde{B}_{\mathrm{p}}(G({\mathrm{\alpha}}), \theta),
\label{math:TG}
\end{equation}
\begin{equation}
G({\mathrm{\alpha}}) = \mathbf{T}_{\mathrm{g}} 
+ B_{\mathrm{g}}(\alpha),
\label{math:G}
\end{equation}
\begin{equation}
\widetilde{B}_{\mathrm{s}}(G({\mathrm{\alpha}}), \beta) = w(G({\mathrm{\alpha}})) B_{\mathrm{s}}(\beta),
\end{equation}
\begin{equation}
\widetilde{B}_{\mathrm{p}}(G({\mathrm{\alpha}}), \theta) = w(G({\mathrm{\alpha}})) B_{\mathrm{p}}(\theta),
\end{equation}
where $G(\alpha)$ denotes a statistical garment model built on top of the body template $\mathbf{T}_{\mathrm{b}}$ (i.e., canonical space). $\mathbf{T}_{\mathrm{g}} \in \mathbb{R}^{N_{\mathrm{G}} \times 3}$ is a garment template with $N_{\mathrm{G}}$ vertices. We define an independent T-posed garment template $\mathbf{T}_{\mathrm{g}}$ for each garment category.
$B_{\mathrm{g}}(\alpha) \in \mathbb{R}^{N_{\mathrm{G}} \times 3}$ models the \textit{Garment Shape Blend Shapes} (GSBS) in canonical space, while $\alpha \in \mathbb{R}^{32}$ is the PCA coefficients that control the GSBS. $\widetilde{B}_{\mathrm{s}}(\cdot) \in \mathbb{R}^{N_{\mathrm{G}} \times 3}$ and $\widetilde{B}_{\mathrm{p}}(\cdot) \in \mathbb{R}^{N_{\mathrm{G}} \times 3}$ are the corresponding garment displacements influenced by the BSBS and BPBS of the body, respectively. $w(\cdot) \in \mathbb{R}^{N_{\mathrm{G}} \times N_{\mathrm{B}}}$ is a weighted matrix that can be computed by searching the KNN (K-Nearest Neighbors) body vertices for each garment vertex~\cite{patel20tailornet,santesteban2019learning} or decoded by a trained neural network~\cite{santesteban2021self,li2022dig}.

\paragraph{Garment, Body, and Camera Estimation.} We use a CNN encoder to map the input image to the garment parametric space and obtain $G(\alpha)$ through Eq.~\ref{math:G}. To build the GSBS and GPBS, we utilize the well-established PyMAF~\cite{pymaf2021,pymafx2023} to predict $\beta$ and $\theta$, and derive $T_{\mathrm{G}}(\alpha, \beta, \theta)$ using Eq.~\ref{math:TG}. Note that the cameras predicted by PyMAF are also subsequently used in modeling meso-scale deformation.

\input{figures/fig_pipeline}

\subsection{Meso-Scale Deformations Modeling}
\label{sec:method_sd}

\paragraph{Pose-Dependent Meso-Scale Deformations (PD-MSD)} To pose the vertices of a body, SMPL uses \textit{Linear Blend Skinning} (LBS) to deform a rigged template. The mapping can be summarized as the following equation:
\begin{equation}
M_{\mathrm{B}}(\beta, \theta) = W\left(T_{\mathrm{B}}(\beta, \theta), J(\beta), \theta, \mathcal{W}\right),
\end{equation}
where $W(\cdot)$ is a skinning function with skinning weights $\mathcal{W} \in \mathbb{R}^{N_{\mathrm{B}} \times 24}$, joint locations $J(\beta) \in \mathbb{R}^{24 \times 3}$, and pose parameters $\theta$ that rig an unposed body mesh $T_{\mathrm{B}}(\beta, \theta)$. 
% To get an initial coarse deformation for garments $\theta$, 
Inspired by~\cite{santesteban2021self,li2022dig}, we extend the SMPL skinning procedure to model the pose-dependent meso-scale deformation (i.e., clothing deformation caused by SMPL pose) by
\begin{equation}
M_{\mathrm{P}}(\alpha, \beta, \theta) = W\left(T_{\mathrm{G}}(\alpha, \beta, \theta), J(\beta), \theta, \widetilde{\mathcal{W}}\right),
\label{math:MP}
\end{equation}
\begin{equation}
\widetilde{\mathcal{W}} = w(G({\mathrm{\alpha}})) \mathcal{W},
\end{equation}
where $\widetilde{\mathcal{W}} \in \mathbb{R}^{N_{\mathrm{G}} \times 24}$ represents the garment skinning weights extended from SMPL.

\paragraph{Pose-Independent Meso-Scale Deformations (PI-MSD)} However, only extending human LBS to garments cannot capture the entire complex meso-scale deformation of clothing. PD-MSD only gives an initial coarse deformation for garments that roughly fit the input image. To accurately reconstruct garments from images, we propose to adopt image diffusion models~\cite{saharia2022image,saharia2022palette} to capture PI-MSD. Given a posed garment model $M_{\mathrm{P}}$, we first project it onto 2D feature maps using the camera predicted by PyMAF in Sec.~\ref{sec:method_tg} to extract local features. Since garments are topological-consistent within different categories, these local features can be mapped and interpolated into UV space to get UV feature maps. Then a conditional diffusion process is performed in UV space to denoise a noisy map and generate a position map. Specifically, our conditional diffusion model is in the form of $p(\boldsymbol{g} \mid \boldsymbol{x})$, where $\boldsymbol{x}$ is the UV feature maps of an image, and $\boldsymbol{g}$ is the position map of a garment. Given a training output position map $\boldsymbol{g}$, we generate a noisy version $\widetilde{\boldsymbol{g}}$, and train a neural network $f$ to denoise $\widetilde{\boldsymbol{g}}$ given UV feature maps $\boldsymbol{x}$ and a noise level indicator $\gamma$, for which the loss is,
\begin{equation}
\mathbb{E}_{(\boldsymbol{x}, \boldsymbol{g})} \mathbb{E}_{\boldsymbol{\epsilon} \sim \mathcal{N}(0, I)} \mathbb{E}_{\gamma}\left\|f(\boldsymbol{x}, \underbrace{\sqrt{\gamma} \boldsymbol{g}+\sqrt{1-\gamma} \boldsymbol{\epsilon}}_{\widetilde{\boldsymbol{g}}}, \gamma)-\boldsymbol{\epsilon}\right\|_{p}^{p}.
\end{equation}
In our experiments, we perform the denoising diffusion process at $64 \times 64$ resolution and use the L1 norm, i.e., $p=1$. The position map $\hat{\boldsymbol{g}}$ predicted by $f$ can be subsequently remapped back to 3D space to the final garment $M_{\mathrm{G}}$.

==> paper/06_application.tex <==
\section{Applications}
\label{sec:application}

\subsection{Surface Details Enhancement}
\label{sec:application_detail}
Various works~\cite{zheng2019deephuman,saito2020pifuhd,xiu2022icon,xiu2023econ,jiang2022selfrecon,qiu2023recmv} show that a high-quality normal map significantly helps to recover geometric details, benefiting from the excellent performance of normal estimators. In this application, we demonstrate that geometric details from normal maps can be integrated into the clothing predicted by \methodName through optimization. Specifically, we first estimate front and back normal maps with ICON's well-trained estimator~\cite{xiu2022icon}. Then we perform iterative optimization via differentiable rendering under the constraints of normals and masks. Fig.~\ref{fig:sde} provides some examples of geometric details enhancement. Alternatively, we can transfer surface details from clothed humans~\cite{xiu2022icon,xiu2023econ} to garments generated by MesoCloth, forming independent clothes with geometric details. Fig.~\ref{fig:app_sde2} provides some examples of carving geometric details from clothed humans produced by ECON~\cite{xiu2023econ} onto garments reconstructed by \methodName.

\paragraph{Discussion.} \textit{Why not model meso-scale deformation and geometric details together? } The reason can be attributed to two factors: 1) Labor intensity. Unlike modeling global meso-scale deformation, sculpting geometric details is often a laborious task, which may take hours, even for expert modelers; 2) Misalignment. Although ControlNet and T2I-Adapter perform well in generating images with correct global meso-scale deformations, it is challenging for them to produce images containing precise fine-grained geometric details aligned with 3D garments. We have constructed some 3D garments with geometric details and conducted experiments on this. \textit{Please refer to the Supplementary for details.}

\subsection{Meso-Scale Deformations Transfer}
Deformation transfer~\cite{sumner2004deformation} is a classic task in computer graphics, aiming to apply the deformation exhibited by a source mesh onto a different target mesh. Pose estimation from images or frames significantly reduces the cost of pose transfer. The estimated human poses can be transferred to an arbitrary virtual avatar by registering SMPL to the avatar~\cite{song20213d,song2023unsupervised,luo2023rabit}. Similarly, the garment meso-scale deformation reconstructed by \methodName can also be transferred to any registered garment, lowering modelers' workload for deforming clothing. Specifically, we can first register our T-pose garment model to a well-designed T-pose cloth and then transfer the reconstructed meso-scale deformation to the target garment. Please refer to the supplementary materials for more details. Fig.~\ref{fig:dt} provides an example of meso-scale deformation transfer.


\subsection{Text-Based Garment Editing}
Recently, text-to-3D generation has achieved remarkable progress~\cite{poole2022dreamfusion,metzer2022latent,hong2022avatarclip,cao2023dreamavatar,zhenyu2023text2tex,richardson2023texture,michel2022text2mesh}, propelled by advancements in large pretrained models~\cite{radford2021learning,girdhar2023imagebind}, text-to-image models~\cite{rombach2022high,ramesh2022hierarchical,saharia2022photorealistic}, and extensive training datasets~\cite{schuhmann2021laion,schuhmann2022laion}. Various works utilize either a basic shape or an SMPL body for initialization and apply text-conditioned editing to generate novel shapes~\cite{metzer2022latent,michel2022text2mesh}, avatars~\cite{hong2022avatarclip,cao2023dreamavatar}, and textures~\cite{zhenyu2023text2tex,richardson2023texture}. Inspired by this, one potential paradigm for clothing design is: 1) reconstructing initial garments with \methodName; 2) generating geometric details using text2mesh~\cite{michel2022text2mesh}; 3) creating UV textures through TEXTure~\cite{richardson2023texture}. Fig.~\ref{fig:te} illustrates two examples of this paradigm.

\subsection{Sketch-Based Garment Editing.} 
We have shown how to enhance garments reconstructed by \methodName using text-to-3D techniques in the main paper. Additionally, garments recovered by \methodName can also be edited through sketch-based modeling approaches~\cite{li2018robust,li2017bendsketch,luo2021simpmodeling,luo2023sketchmetaface}. We conduct an experiment on adopting the strategy proposed by SimpModeling~\cite{luo2021simpmodeling} to sketch-based garment editing. Specifically, given a garment reconstructed by \methodName, we render its 2D sketch, as well as the front and back view depth maps. Subsequently, we modify the 2D sketch (e.g., adding strokes to depict geometric details) and learn a pixel-aligned implicit field~\cite{saito2019pifu,chibane2020neural,qiu2023recmv} from the refined sketch and the rendered depth maps. Fig.~\ref{fig:app_sbe} illustrates some examples of sketch-based garment editing.


==> supp_figures/fig_ablation2.tex <==
\begin{figure*}[htbp]
  \centering
  \includegraphics[width=.93\linewidth]{images/fig_compare2.png}
  \caption{Qualitative comparison between our method and the optional strategies for modeling pose-independent meso-scale deformation. For each case, the input image (a) is followed by the results generated by (b) the displacement-based method, (c) the feature-line-based method, and (d) our method.}
  \label{fig:data_ablation2}
\end{figure*}

==> supp_figures/fig_app_sbe.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=.99\linewidth]{supp_images/fig_sk.png}
  \caption{An illustration of sketch-based garment editing. Given a garment  (a) reconstructed by \methodName, we can further sculpt geometric details (c) onto it with a detailed sketch (b).}
  \label{fig:app_sbe}
\end{figure}

==> supp_figures/fig_app_sde2.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=.90\linewidth]{supp_images/fig_sde2.png}
  \caption{Examples of transferring surface details from clothed humans produced by ECON~\cite{xiu2023econ} to garments reconstructed by \methodName.}
  \label{fig:app_sde2}
\end{figure}

==> supp_figures/fig_data_template.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=.98\linewidth]{supp_images/fig_template_f322.png}
  \caption{Predefined templates for each garment category, including (a) dress, (b) skirt, (c) top, (d) pant, and (e) coat.}
  \label{fig:data_template}
\end{figure}

==> supp_figures/fig_wr_data.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=.98\linewidth]{supp_images/fig_wr_data2.png}
  \caption{Given a T-posed garment (a) in \dataName, artists are required to sculpt geometric details (b) on it. Then these surface details are transferred programmatically to the corresponding garment with meso-scale deformations (c) to obtain the final garment (d).}
  \label{fig:wr_data}
\end{figure}

==> supp_figures/fig_wr_t2i.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=.98\linewidth]{supp_images/fig_wr_t2i.png}
  \caption{Sampled images generated by ControlNet~\cite{zhang2023adding} and T2I-Adapter~\cite{mou2023t2i}. For each row, the 3D garment is followed by four generated images. While these models perform well in generating images with correct global meso-scale deformations, producing images with precise fine-grained geometric details aligned with 3D garments remains challenging.}
  \label{fig:wr_t2i}
\end{figure}

==> supp_figures/fig_wr_training_result.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=.98\linewidth]{supp_images/fig_wr_training2.png}
      \caption{Qualitative comparisons of our method trained on data without geometric details (b) and with geometric details (c).}
  \label{fig:wr_training_result}
\end{figure}

==> supp_tables/table_ablation2.tex <==
\begin{table}[htbp]
    \renewcommand{\arraystretch}{0.8}
    \centering
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{l|c|c|c}
        % \hline 
        \toprule
        Method & Displacement & Feature Lines & Ours \\
        \midrule
        Chamfer-$L_2$ $\downarrow$ & 14.329 & 12.616 & \textbf{7.625} \\
        \midrule
        Normal-Consis. $\uparrow$  & 0.829  & 0.841 & \textbf{0.916} \\
        \bottomrule
        \end{tabular}
    }
    \caption{Quantitative comparison between our method and alternative strategies for modeling pose-independent meso-scale deformation. Our method achieves the best results in terms of Chamfer-$L_2$ and Normal Consistency.}
    \label{tab:ablation2}
    \vspace{-3mm}
\end{table}

==> supp_tables/table_dataset.tex <==
\begin{table}[htbp]
    \renewcommand{\arraystretch}{0.8}
    \centering
    \resizebox{0.49\textwidth}{!}{
        \begin{tabular}{l|c|c|c|c|c}
        % \hline 
        \toprule
        Category & Dress & Coat & Skirt & Top & Pant \\
        \midrule
        Total & 1,571 & 1,427 & 1,049 & 1,501 & 452 \\
        \bottomrule
        \end{tabular}
    }
    \caption{Data statistics for each garment category.}
    \label{tab:dataset}
\end{table}

